P4L: Privacy Preserving Peer-to-Peer Learning for Infrastructureless Setups

Distributed (or Federated) learning enables users to train machine learning models on their very own devices, while they share only the gradients of their models usually in a differentially private way (utility loss). Although such a strategy provides better privacy guarantees than the traditional centralized approach, it requires users to blindly trust a centralized infrastructure that may also become a bottleneck with the increasing number of users. In this paper, we design and implement P4L: a privacy preserving peer-to-peer learning system for users to participate in an asynchronous, collaborative learning scheme without requiring any sort of infrastructure or relying on differential privacy. Our design uses strong cryptographic primitives to preserve both the confidentiality and utility of the shared gradients, a set of peer-to-peer mechanisms for fault tolerance and user churn, proximity and cross device communications. Extensive simulations under different network settings and ML scenarios for three real-life datasets show that P4L provides competitive performance to baselines, while it is resilient to different poisoning attacks. We implement P4L and experimental results show that the performance overhead and power consumption is minimal (less than 3mAh of discharge).

==> figs/figureWall0.tex <==

% \begin{figure*}[!t]
%     \captionsetup[subfloat]%{captionskip=-5pt,nearskip=0pt,farskip=0pt}
%     {}
%     \centering
%     \subfloat[Loss]{
%     \label{figure:crypto_cifar_non_iid_a}
%     \includegraphics[clip=true, trim=0 0 0 0, width=0.3\textwidth]{figs/plain-non-iid-syn-3-10-losses-encryption.tex-crop}
%     }
%     \hspace{0.05mm}
%     \subfloat[Accuracy]{%
%     \label{figure:crypto_cifar_non_iid_b}
%     \includegraphics[clip=true, trim=0 0 0 0, width=0.3\textwidth]{figs/plain-non-iid-syn-3-10-acc-encryption.tex-crop}
%     }
%     \hspace{0.05mm}
%     \subfloat[AUC]{%
%     \label{figure:crypto_cifar_non_iid_c}
%     \includegraphics[clip=true, trim=0 0 0 0, width=0.3\textwidth]{figs/plain-non-iid-syn-3-10-auc-encryption.tex-crop}
%     }
%     \vspace{-0.75em}
%     \caption{Effect of encryption on Loss, Accuracy and AUC on non-IID data for \texttt{CIFAR-10} (\texttt{sz}=3-10, \texttt{mrt}=50, \texttt{mrr}=50).
%     %Legend is the same across all plots.
%     }\vspace{-0.4cm}
%     \label{figure:crypto_cifar_non_iid}
% \end{figure*}

% \begin{figure}[!t]
%     \captionsetup[subfloat]%{captionskip=-5pt,nearskip=0pt,farskip=0pt}
%     {}
%     \centering
%     \subfloat[Loss]{
%     \label{figure:crypto_avito_non_iid_a}
%     \includegraphics[clip=true, trim=0 0 0 0, width=0.235\textwidth]{figs/lg-plain-non-iid-syn-3-10-losses-encryption.tex-crop}
%     }
%     % \hspace{0.15mm}
%     \subfloat[AUC]{%
%     \label{figure:crypto_avito_non_iid_c}
%     \includegraphics[clip=true, trim=0 0 0 0, width=0.235\textwidth]{figs/lg-plain-non-iid-syn-3-10-auc-encryption.tex-crop}
%     }
%     \vspace{-0.75em}
%     \caption{Effect of encryption on Loss and AUC on non-IID data for \texttt{Avito} (\texttt{sz}=3-10, \texttt{mrt}=50, \texttt{mrr}=50).}
%     \label{figure:crypto_avito_non_iid}
%     \vspace{-0.4cm}
% \end{figure}


==> sections/background.tex <==
\section{Building Blocks}
\label{sec:background}

\subsection{Confidentiality}
\label{ssec:confidentiality}
\toolname uses an additively homomorphic encryption scheme to perform \emph{private federated aggregation}. Given an assymetric public-private key-pair $(pk, sk)$, the encryption scheme is defined by three functions: (i) the encrypt function, where given a public key $pk$ and a message $M$, it outputs a ciphertext, $C=Enc(pk, M)$, (ii) the decrypt function, that given a ciphertext and a private key $sk$, it outputs a decrypted message, $P=Dec(sk, M)$. And, finally, the signing function, where given a message $M$ and a secret key $sk$, it outputs a signature on the message, $S=Sign(sk, M)$. The additive homomorphic property guarantees that the addition of two ciphertexts $C1=Enc(pk, M_1)$ and $C2=Enc(pk,M_2)$, encrypted under the same key, results in the addition of the encryption of its messages. Specifically:
\begin{equation*}
    Enc(pk,M_1)+Enc(pk,M_2) = Enc(pk,M1+M2)
\end{equation*}
In our \toolname prototype we use the Paillier partial homomorphic encryption scheme over elliptic curves \cite{10.1007/3-540-48910-X_16}.


==> sections/discussion.tex <==
\section{Limitations}

\subsection{Poisoning attacks}
\notes{ioannis?}
Label flipping attacks~\cite{10.5555/3007337.3007488} 

Backdoor attacks~\cite{chen2017targeted,10.5555/3327757.3327896} from the synergy participants can force users classifier missclassify an image by containing certain pixels or a backdoor key. Defending  against  such  attacks  during  training  is  a  hard  and open problem in the literature.

Comment: The experimental validation is not convincing; The real-world experiments are quite limited (only hundred-scale parameters). It doesn't really validate the promise of the proposed scheme. 
[Minos] This is a h/w limitation that will change in the near future.

Comment: The resiliency to few adversarial attacks does not seem to be an intentional product of your system but more a natural byproduct of any decentralized approach
[Ioannis] To check/address (natural trait of the system).
